Visualizing Distributed Traces in Aggregate

Distributed systems are comprised of many components that communicate together to form an application. Distributed tracing gives us visibility into these complex interactions, but it can be difficult to reason about the system's behavior, even with traces. Systems collect large amounts of tracing data even with low sampling rates. Even when there are patterns in the system, it is often difficult to detect similarities in traces since current tools mainly allow developers to visualize individual traces. Debugging and system optimization is difficult for developers without an understanding of the whole trace dataset. In order to help present these similarities, this paper proposes a method to aggregate traces in a way that groups together and visualizes similar traces. We do so by assigning a few traces that are representative of each set. We suggest that traces can be grouped based on how many services they share, how many levels the graph has, how structurally similar they are, or how close their latencies are. We also develop an aggregate trace data structure as a way to comprehensively visualize these groups and a method for filtering out incomplete traces if a more complete version of the trace exists. The unique traces of each group are especially useful to developers for troubleshooting. Overall, our approach allows for a more efficient method of analyzing system behavior.

==> sections/references.tex <==
\section{References}
\darby{fix this!}

1) Las-Casas, P., Papakerashvili, G., Anand, V., Mace, J.: Sifter: Scalable Sampling for Distributed Traces,
without Feature Engineering.
\url{https://people.mpi-sws.org/~jcmace/papers/lascasas2019sifter.pdf} 

2) Gias, A. UI., Gao, Y., Sheldon, M., Peruspuía, J. A., O'Brien, O., Casale, G.: SampleHST: Efficient On-the-Fly Selection of
Distributed Traces. In arXiv 2022. \url{https://arxiv.org/abs/2210.04595} 

3) Huang, L., Zhu, T.: tprof: performance profiling via structural aggregation and automated analysis of distributed systems traces. In: SoCC 2021, pp. 76–91. \url{https://dl.acm.org/doi/10.1145/3472883.3486994} 

4) Huye, D., Shkuro, Y., Sambasivan, R. R.: Lifting the veil on Meta’s microservice architecture: Analyses of topology and request workflows. In: USENIX ATC 2023, pp. 419–432. \url{https://www.usenix.org/conference/atc23/presentation/huye} 

5) Wu, Y., Chen, A., Phan, L. T. X.: Zeno: Diagnosing Performance Problems
with Temporal Provenance. In: NSDI 2019, pp. 395-420. \url{https://www.usenix.org/system/files/nsdi19-wu.pdf} 

6) Connected Components in an Undirected Graph. In GeeksForGeeks. \url{https://www.geeksforgeeks.org/connected-components-in-an-undirected-graph/} 

